Deep Global Registration

We present Deep Global Registration, a differentiable framework for pairwise registration of real-world 3D scans. Deep global registration is based on three modules: a 6-dimensional convolutional network for correspondence confidence prediction, a differentiable Weighted Procrustes algorithm for closed-form pose estimation, and a robust gradient-based SE(3) optimizer for pose refinement. Experiments demonstrate that our approach outperforms state-of-the-art methods, both learning-based and classical, on real-world data.

==> assets/3dmatch/2_5cm.tex <==
\begin{table}
\centering
\small
\caption{Registration results on point clouds voxelized with 2.5cm voxel size.}\label{tab:2.5cm}
\resizebox{0.995\linewidth}{!}{
\begin{tabular}{c||c|c|c|c}
    \hline
     & Recall & RTE (cm) & RRE (deg) & Time (s) \\
    \hline
    Ours                       & \textbf{79.0}\% & \textbf{7.20} & \textbf{2.23} & 2.33 \\    
    RANSAC~\cite{rusu2009icra} & 46.3\% & 8.05 & 2.66 & 3.22 \\ 
    FGR~\cite{zhou2016eccv}    & 30.7\% & 11.5 & 4.79 & \textbf{1.63} \\
    \hline
\end{tabular}
}
\end{table}

==> assets/3dmatch/3dmatch_pair.tex <==
\begin{table}[ht]
\centering
\caption{Pairwise registration: Translation Error (TE), Rotation Error (RE), and registration recall on the 3DMatch benchmark~\cite{zeng20163dmatch}. A pair is successfully registered if the predicted rotation $<$ 15${}^\circ$ and translation $<$ 30cm. RE in degree ($^\circ$) and TE in cm. RANSAC-4M denotes RANSAC with maximum 4M iterations. \textit{Note: Go-ICP works much slower on most scenes without perfect overlaps.}}\label{table:3dmatch}




\begin{tabular}{c|c|c|c|c}
                 & Recall & RTE & RRE & time \\
                 \hline
    Ours-5cm     & 76.2\% & 8.54 & 2.77 & 1.61 \\
    RANSAC-5cm   & 70.7\% & 9.16 & 2.95 & 2.32 \\
    FGR-5cm      & 42.7\% & 10.6 & 4.08 & 0.31     
\end{tabular}


\begin{tabular}{c|c|c|c|c}
                 & Recall & RTE & RRE & time \\
                 \hline
    ICP (point-to-point)   & 6.04\% & 18.1 & 8.25 & 0.25 \\    
    ICP (point-to-plane)   & 6.59\% & 15.2 & 6.61 & 0.27 \\    
    Go-ICP                 & 22.9\% & 14.7 & 5.38 & 771.0 \\
    DCP                    & 3.22\% & 21.4 & 8.42 & 0.07 \\    
    PointNetLK             & 1.61\% & 21.3 & 8.04 & 0.12
\end{tabular}

\end{table}
\footnote{Go-ICP was measured on a Intel i7-5820K@3.3GHz CPU with a single thread. All the other methods were measured on Intel i7-7700@3.6GHz CPU. Learning based methods were evaluated with an NVIDIA GTX 1080 Ti in addition.}



==> assets/3dmatch/3dmatch_pair_table.tex <==
\begin{table*}[ht]
\centering
\caption{Pairwise registration: Translation Error (TE), Rotation Error (RE), and registration recall on the 3DMatch benchmark~\cite{zeng20163dmatch}. A pair is successfully registered if the predicted rotation $<$ 15${}^\circ$ and translation $<$ 30cm. RE in degree ($^\circ$) and TE in cm. RANSAC-4M denotes RANSAC with maximum 4M iterations. \textit{Note: Go-ICP works much slower on most scenes without perfect overlaps.}}\label{table:3dmatch}

\resizebox{0.995\linewidth}{!}{
    \begin{tabular}{l||lll|lll|lll|lll|lll|lll} 
    \toprule
            & \multicolumn{3}{c|}{ICP (point-to-plane)} & \multicolumn{3}{c|}{ICP (point-to-point)}  & \multicolumn{3}{c|}{Go-ICP} & \multicolumn{3}{c|}{FGR-5cm~\cite{zhou2016eccv}}   & \multicolumn{3}{c|}{RANSAC-5cm-4M} & \multicolumn{3}{c}{Ours-5cm\todo{training}} \\ \hline
            & TE & RE & Recall & TE & RE & Recall   & TE  & RE  & Recall   & TE   & RE  & Recall & TE  & RRE  & Recall   & TE   & RE  & Recall \\
    \midrule
    Kitchen & 18.9 & 7.36 & 4.35\%    & 19.5 & 8.38 & 4.35\%    & 15.1 & 5.67 & 28.1\%    &  9.46 & 4.07 & 45.7\%     & 7.97 & 2.81 & 73.1\%       &  6.46 & 2.25 & 85.38\% \\
    Home 1  & 12.6 & 5.82 & 8.97\%    & 17.7 & 6.42 & 8.33\%    & 14.2 & 4.84 & 19.9\%    &  8.36 & 3.07 & 50.6\%     & 9.88 & 2.83 & 79.5\%       &  7.05 & 2.13 & 81.41\% \\
    Home 2  & 12.6 & 5.34 & 7.69\%    & 16.5 & 7.87 & 9.13\%    & 12.9 & 4.55 & 24.5\%    &  9.09 & 3.82 & 38.5\%     & 9.02 & 3.63 & 63.0\%       &  8.19 & 2.92 & 64.90\% \\
    Hotel 1 & 14.1 & 8.01 & 5.31\%    & 19.1 & 9.30 & 4.42\%    & 14.9 & 6.28 & 19.0\%    & 10.61 & 3.70 & 45.6\%     & 9.27 & 3.16 & 83.6\%       &  7.31 & 2.42 & 90.27\% \\
    Hotel 2 & 11.2 & 3.42 & 3.84\%    & 23.4 & 10.7 & 1.92\%    & 15.5 & 6.66 & 23.1\%    & 12.48 & 4.85 & 37.5\%     & 9.86 & 3.15 & 75.0\%       &  6.67 & 2.30 & 75.96\% \\
    Hotel 3 & 23.8 & 1.85 & 3.70\%    & 27.4 & 6.52 & 5.56\%    & 11.7 & 5.84 & 22.2\%    & 11.86 & 4.39 & 48.1\%     & 8.55 & 2.92 & 75.9\%       &  5.99 & 1.98 & 72.22\% \\
    Study   & 16.2 & 8.84 & 8.22\%    & 16.3 & 11.1 & 6.16\%    & 15.7 & 4.80 & 14.7\%    & 13.35 & 4.74 & 27.7\%     & 9.86 & 2.68 & 61.0\%       &  10.52 & 2.97 & 69.18\% \\
    Lab     & 14.2 & 4.09 & 16.9\%    & 17.3 & 5.18 & 14.3\%    & 15.0 & 4.02 & 32.5\%    &  9.60 & 4.03 & 48.1\%     & 8.84 & 2.41 & 54.5\%       &  8.53 & 1.97 & 70.13\% \\ \hline
    Average & 15.2 & 6.61 & 6.59\%    & 18.1 & 8.25 & 6.04\%    & 14.7 & 5.38 & 22.9\%    & 10.60 & 4.08 & 42.7\%     & 9.16 & 2.95 & 70.7\%       &  7.59 & 2.37 & 76.18\% \\
    \hline
    Avg. Runtime  & \multicolumn{3}{c|}{0.271 sec} & \multicolumn{3}{c|}{0.249 sec} & \multicolumn{3}{c|}{771 sec} & \multicolumn{3}{c|}{0.31 sec}   & \multicolumn{3}{c|}{2.32 sec} & \multicolumn{3}{c}{1.61 sec} \\
    \bottomrule
    \end{tabular}
}

\resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l||lll|lll|lll|lll|lll} 
    \toprule
           & \multicolumn{3}{c|}{FGR-2.5cm~\cite{zhou2016eccv}}  & \multicolumn{3}{c|}{RANSAC-2.5cm-4M} & \multicolumn{3}{c|}{DCP~\cite{wang2019deep}} & \multicolumn{3}{c|}{PointNetLK~\cite{aoki2019pointnetlk}} & \multicolumn{3}{c}{Ours-2.5cm} \\ \hline
          & RTE   & RRE  & Recall & RTE  & RRE  & Recall   & RTE   & RRE  & Recall   & RTE   & RRE  & Recall & RTE & RRE & Recall\\
    \midrule
    Kitchen &  11.2 & 4.73 & 37.2\%     & 6.59 & 2.47 & 45.1\%   & 24.1 & 8.38 & 2.57\%   & 22.5 & 8.41 & 1.98\% & 6.22 & 2.05 & 84.8\% \\
    Home 1  &  10.7 & 4.63 & 46.8\%     & 7.85 & 2.42 & 64.7\%   & 19.0 & 6.73 & 2.56\%   & 21.6 & 5.09 & 1.92\% 
    & 6.86 & 2.05 & 85.3\% \\
    Home 2  &  8.80 & 3.79 & 34.1\%     & 7.19 & 2.46 & 49.0\%   & 23.1 & 8.55 & 4.33\%   & 15.3 & 8.35 & 2.40\% & 7.67 & 2.75 & 74.0\% \\
    Hotel 1 & 11.1 & 4.57 & 32.3\%     & 7.78 & 2.57 & 49.6\%   & 22.7 & 8.79 & 0.88\%    & 20.5 & 7.00 & 0.88\% & 6.77 & 2.16 & 85.0\% \\
    Hotel 2 & 13.8 & 6.06 & 26.9\%     & 9.02 & 3.20 & 47.1\%   & 17.4 & 8.88 & 0.96\%    & - & - & 0 & 6.11 & 2.25 & 78.8\% \\
    Hotel 3 & 13.6 & 7.69 & 27.8\%     & 7.84 & 2.86 & 64.8\%   & 23.9 & 14.3 & 1.85\%    & 27.4 & 13.9 & 1.85\% & 6.42 & 2.05 & 81.5\% \\
    Study   & 15.9 & 5.44 & 16.1\%     & 9.17 & 2.93 & 29.1\%   & 21.2 & 11.1 & 3.77\%  & 26.8 & 8.96 & 1.37\%   & 9.96 & 2.69 & 75.3\% \\
    Lab     & 11.3 & 4.49 & 46.8\%     & 8.10 & 2.65 & 42.9\%    & 19.7 & 4.94 & 10.4\%  & 22.5 & 8.02 & 3.90\%   & 7.57 & 1.88 & 67.5\% \\ \hline
    Average & 11.5 & 4.79 & 30.7\%     & 8.05 & 2.66 & 46.3\%   & 21.4 & 8.42 & 3.22\%   & 21.3 & 8.04 & 1.61\%  & 7.20 & 2.23 & 79.0\% \\
    \hline
    Avg. Runtime & \multicolumn{3}{c|}{1.63 sec}  & \multicolumn{3}{c|}{3.22 sec} & \multicolumn{3}{c|}{0.07 sec} &\multicolumn{3}{c|}{0.12 sec} & \multicolumn{3}{c}{2.33 sec} \\
    \bottomrule
    \end{tabular}
}
\end{table*}
\footnote{Go-ICP was measured on a Intel i7-5820K@3.3GHz CPU with a single thread. All the other methods were measured on Intel i7-7700@3.6GHz CPU. Learning based methods were evaluated with an NVIDIA GTX 1080 Ti in addition.}



==> assets/3dmatch/icp_and_learning.tex <==
\begin{table}
\centering
\small
\caption{Results of ICP variants and learning-based methods on real-world scans. With low recall rates, these methods generally fail on real-world scans.}\label{tab:icp-learning}
\resizebox{0.995\linewidth}{!}{
\begin{tabular}{c||c|c|c|c}
    \hline
     & Recall & TE (cm) & RE (deg) & Time (s) \\
    \hline
    DCP~\cite{wang2019deep}              & 3.22\% & 21.4 & 8.42 & 0.07 \\    
    PointNetLK~\cite{aoki2019pointnetlk} & 1.61\% & 21.3 & 8.04 & 0.12 \\    
    ICP (P2Point)~\cite{Zhou2018}        & 6.04\% & 18.1 & 8.25 & 0.25 \\    
    ICP (P2Plane)~\cite{Zhou2018}        & 6.59\% & 15.2 & 6.61 & 0.27 \\    
    Go-ICP~\cite{yang2015go}             & 22.9\% & 14.7 & 5.38 & 771.0 \\
    Super4PCS~\cite{mellado2014super}    & 21.6\% & 14.1 & 5.25 & 4.55\\
    \hline
\end{tabular}
}
\vspace*{-1em}
\end{table}

==> assets/modelnet40/cropped.tex <==
\begin{table}[h]
\centering
\label{table:registration-non-cropped}
\caption{Partial scan to model registration}
\resizebox{0.995\linewidth}{!}{
    \begin{tabular}{l||c|c|c|c||c}
    \hline
    & FGR ~\cite{Zhou2018} & RANSAC ~\cite{Zhou2018} & DCP~\cite{wang2019deep} & PointNetLK~\cite{aoki2019pointnetlk} & Ours \\
    \hline
    RTE (mm) & 27.97 & 21.52 & 74.31 & 58.14 & 42.96 \\
    RRE (deg) & 4.94 & 3.17 & 7.57 & 5.89 & 4.11 \\
    Recall & 45.44\% & 75.19\% & 29.30\% & 10.31\% & 61.14\% \\
    Time & 0.19 & 1.89 & 0.04 & 0.08 & 2.02 \\
    \hline
    \end{tabular}
}
\end{table}

==> assets/modelnet40/non_cropped.tex <==
\begin{table}[h]
\centering
\label{table:registration-non-cropped}
\caption{Complete model-to-model registration}
\resizebox{0.995\linewidth}{!}{
    \begin{tabular}{l||c|c|c|c||c}
    \hline
    & FGR ~\cite{Zhou2018} & RANSAC ~\cite{Zhou2018} & DCP~\cite{wang2019deep} & PointNetLK~\cite{aoki2019pointnetlk} & Ours \\
    \hline
    RTE (mm) & 11.31 & 7.68 & 3.36 & 0.34 & 5.65 \\
    RRE (deg) & 3.36 & 1.67 & 2.03 & 0.98 & 1.17 \\
    Recall & 53.14\% & 82.03\% & 99.96\% & 24.22\% & 90.47\% \\
    Time & 0.26 & 1.74 & 0.038 & 0.068 & 2.43 \\
    \hline
    \end{tabular}
}
\end{table}
